Self-Concordant Analysis of Generalized Linear Bandits with Forgetting

Contextual sequential decision problems with categorical or numerical observations are ubiquitous and Generalized Linear Bandits (GLB) offer a solid theoretical framework to address them. In contrast to the case of linear bandits, existing algorithms for GLB have two drawbacks undermining their applicability. First, they rely on excessively pessimistic concentration bounds due to the non-linear nature of the model. Second, they require either non-convex projection steps or burn-in phases to enforce boundedness of the estimators. Both of these issues are worsened when considering non-stationary models, in which the GLB parameter may vary with time. In this work, we focus on self-concordant GLB (which include logistic and Poisson regression) with forgetting achieved either by the use of a sliding window or exponential weights. We propose a novel confidence-based algorithm for the maximum-likehood estimator with forgetting and analyze its perfomance in abruptly changing environments. These results as well as the accompanying numerical simulations highlight the potential of the proposed approach to address non-stationarity in GLB.

==> conclusion.tex <==

{ \color{purple}
\section{CONCLUSION}
We have shown that the MLE with forgetting is sufficient to obtain 
theoretical guarantees for GLBs in non-stationary environments. 
Enforcing boundedness of the MLE is a strong requirement in GLBs analysis.
While, in stationary environments, a burning phase may permit to avoid the use of a projection step ensuring the boundedness of the estimator, this is no longer the case in abruptly changing environments. 
The approach presented here circumvents the need for a projection by exploiting the self-concordance property of the inverse link function. 
By extending previous concentration results to the more general \textit{weighted} MLE,
we also reduce the dependency on a \textit{key problem-dependent constant} arising 
from the non-linear nature of GLMs.
This has consequences both on the design of our algorithm and on the regret analysis.
As a side product, our analysis shows that self-concordant GLB can be analyzed without projecting the MLE onto the admissible parameter space, whether the environment is stationary or not.
}
\clearpage
